BBC-Oxford British Sign Language Dataset

In this work, we introduce the BBC-Oxford British Sign Language (BOBSL) dataset, a large-scale video collection of British Sign Language (BSL). BOBSL is an extended and publicly released dataset based on the BSL-1K dataset introduced in previous work. We describe the motivation for the dataset, together with statistics and available annotations. We conduct experiments to provide baselines for the tasks of sign recognition, sign language alignment, and sign language translation. Finally, we describe several strengths and limitations of the data from the perspectives of machine learning and linguistics, note sources of bias present in the dataset, and discuss potential applications of BOBSL in the context of sign language technology. The dataset is available at https://www.robots.ox.ac.uk/~vgg/data/bobsl/.

==> 08-public-protocols.tex <==
\section{Evaluation server} \label{sec:public-evaluation-protocols}

We make available public evaluation protocols available
on the CodaLab platform to support community
progress on automatic sign understanding tasks.
See the project page~\cite{bobsl21} for details.

